Visualization for Trust in Machine Learning Revisited: The State of the Field in 2023

Visualization for explainable and trustworthy machine learning remains one of the most important and heavily researched fields within information visualization and visual analytics with various application domains, such as medicine, finance, and bioinformatics. After our 2020 state-of-the-art report comprising 200 techniques, we have persistently collected peer-reviewed articles describing visualization techniques, categorized them based on the previously established categorization schema consisting of 119 categories, and provided the resulting collection of 542 techniques in an online survey browser. In this survey article, we present the updated findings of new analyses of this dataset as of fall 2023 and discuss trends, insights, and eight open challenges for using visualizations in machine learning. Our results corroborate the rapidly growing trend of visualization techniques for increasing trust in machine learning models in the past three years, with visualization found to help improve popular model explainability methods and check new deep learning architectures, for instance.

==> latexmkrc <==
# See https://www.overleaf.com/learn/latex/Articles/How_to_use_latexmkrc_with_Overleaf 
# and https://www.overleaf.com/learn/latex/Articles/Using_Latexdiff_For_Marking_Changes_To_Tex_Documents
# and https://shannonmlocke.wordpress.com/2020/05/10/a-short-guide-to-using-latexdiff/

# Generate the highlighted diff PDF for the major revision, unless a particular file (such as a revision cover letter, for instance) is selected
# Also consider the "flatten" option for latexdiff, in case of multiple files
if (!($ARGV[-1] =~ /letter_of_amendments/)) {
# Comment out the line below to stop generating the color-highlighted diff version
# Does not really work for this project due to abundance of inline math ($ ... $) TeX commands that are not processed well by latexdiff :(
#$pdflatex = "latexdiff -t UNDERLINE --disable-citation-markup --no-links --config='PICTUREENV=(?:picture|DIFnomarkup|align|tabular|figure)[\w\d*@]*' TrustMLVis-initial-submission.tex TrustMLVis.tex > main-diff.tex; pdflatex %O main-diff";
} else {
  $pdflatex = 'pdflatex  %O  --shell-escape %S';
}
